Unveiling Anomalous Edges and Nominal Connectivity of Attributed Networks

Uncovering anomalies in attributed networks has recently gained popularity due to its importance in unveiling outliers and flagging adversarial behavior in a gamut of data and network science applications including {the Internet of Things (IoT)}, finance, security, to list a few. The present work deals with uncovering anomalous edges in attributed graphs using two distinct formulations with complementary strengths, which can be easily distributed, and hence efficient. The first relies on decomposing the graph data matrix into low rank plus sparse components to markedly improve performance. The second broadens the scope of the first by performing robust recovery of the unperturbed graph, which enhances the anomaly identification performance. The novel methods not only capture anomalous edges linking nodes of different communities, but also spurious connections between any two nodes with different features. Experiments conducted on real and synthetic data corroborate the effectiveness of both methods in the anomaly identification task.

==> figures/Figexample.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp11872831081545843] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (94,122.75) .. controls (94,116.26) and (99.26,111) .. (105.75,111) .. controls (112.24,111) and (117.5,116.26) .. (117.5,122.75) .. controls (117.5,129.24) and (112.24,134.5) .. (105.75,134.5) .. controls (99.26,134.5) and (94,129.24) .. (94,122.75) -- cycle ;
%Shape: Circle [id:dp8707186597008119] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (108,168.75) .. controls (108,162.26) and (113.26,157) .. (119.75,157) .. controls (126.24,157) and (131.5,162.26) .. (131.5,168.75) .. controls (131.5,175.24) and (126.24,180.5) .. (119.75,180.5) .. controls (113.26,180.5) and (108,175.24) .. (108,168.75) -- cycle ;
%Shape: Circle [id:dp19716879453124414] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (145,125.75) .. controls (145,119.26) and (150.26,114) .. (156.75,114) .. controls (163.24,114) and (168.5,119.26) .. (168.5,125.75) .. controls (168.5,132.24) and (163.24,137.5) .. (156.75,137.5) .. controls (150.26,137.5) and (145,132.24) .. (145,125.75) -- cycle ;
%Shape: Circle [id:dp5421240585147511] 
\draw  [fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=1 ] (163,67.75) .. controls (163,61.26) and (168.26,56) .. (174.75,56) .. controls (181.24,56) and (186.5,61.26) .. (186.5,67.75) .. controls (186.5,74.24) and (181.24,79.5) .. (174.75,79.5) .. controls (168.26,79.5) and (163,74.24) .. (163,67.75) -- cycle ;
%Shape: Circle [id:dp5266517161511364] 
\draw  [fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=1 ] (184.75,41.25) .. controls (184.75,34.76) and (190.01,29.5) .. (196.5,29.5) .. controls (202.99,29.5) and (208.25,34.76) .. (208.25,41.25) .. controls (208.25,47.74) and (202.99,53) .. (196.5,53) .. controls (190.01,53) and (184.75,47.74) .. (184.75,41.25) -- cycle ;
%Shape: Circle [id:dp7250495590470001] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (187,156.75) .. controls (187,150.26) and (192.26,145) .. (198.75,145) .. controls (205.24,145) and (210.5,150.26) .. (210.5,156.75) .. controls (210.5,163.24) and (205.24,168.5) .. (198.75,168.5) .. controls (192.26,168.5) and (187,163.24) .. (187,156.75) -- cycle ;
%Shape: Circle [id:dp9497674678673771] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (213.75,126.25) .. controls (213.75,119.76) and (219.01,114.5) .. (225.5,114.5) .. controls (231.99,114.5) and (237.25,119.76) .. (237.25,126.25) .. controls (237.25,132.74) and (231.99,138) .. (225.5,138) .. controls (219.01,138) and (213.75,132.74) .. (213.75,126.25) -- cycle ;
%Shape: Circle [id:dp24101502681641018] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (237.75,160) .. controls (237.75,153.51) and (243.01,148.25) .. (249.5,148.25) .. controls (255.99,148.25) and (261.25,153.51) .. (261.25,160) .. controls (261.25,166.49) and (255.99,171.75) .. (249.5,171.75) .. controls (243.01,171.75) and (237.75,166.49) .. (237.75,160) -- cycle ;
%Straight Lines [id:da9543557986424249] 
\draw    (105.75,134.5) -- (119.75,157) ;
%Straight Lines [id:da10929190433831026] 
\draw    (105.75,134.5) -- (144.5,131) ;
%Straight Lines [id:da25650819959024296] 
\draw    (144.5,131) -- (119.75,157) ;
%Straight Lines [id:da923722529770429] 
\draw    (156.75,114) -- (174.75,79.5) ;
%Straight Lines [id:da22702981177511483] 
\draw    (167.5,132) -- (189.5,148) ;
%Straight Lines [id:da6576453166269782] 
\draw    (184.5,60) -- (196.5,53) ;
%Straight Lines [id:da229908490344773] 
\draw    (211.5,71) -- (196.5,53) ;
%Shape: Circle [id:dp9435597803943747] 
\draw  [fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=1 ] (205,77.75) .. controls (205,71.26) and (210.26,66) .. (216.75,66) .. controls (223.24,66) and (228.5,71.26) .. (228.5,77.75) .. controls (228.5,84.24) and (223.24,89.5) .. (216.75,89.5) .. controls (210.26,89.5) and (205,84.24) .. (205,77.75) -- cycle ;
%Straight Lines [id:da3496686734009835] 
\draw    (205.5,148) -- (225.5,138) ;
%Straight Lines [id:da5285856080168552] 
\draw    (225.5,138) -- (237.75,160) ;
%Straight Lines [id:da07333688319306009] 
\draw    (207.5,162) -- (237.75,160) ;
%Shape: Circle [id:dp5269971345201871] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (319,118.75) .. controls (319,112.26) and (324.26,107) .. (330.75,107) .. controls (337.24,107) and (342.5,112.26) .. (342.5,118.75) .. controls (342.5,125.24) and (337.24,130.5) .. (330.75,130.5) .. controls (324.26,130.5) and (319,125.24) .. (319,118.75) -- cycle ;
%Shape: Circle [id:dp9720115581100084] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (333,164.75) .. controls (333,158.26) and (338.26,153) .. (344.75,153) .. controls (351.24,153) and (356.5,158.26) .. (356.5,164.75) .. controls (356.5,171.24) and (351.24,176.5) .. (344.75,176.5) .. controls (338.26,176.5) and (333,171.24) .. (333,164.75) -- cycle ;
%Shape: Circle [id:dp8115609521023355] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (370,121.75) .. controls (370,115.26) and (375.26,110) .. (381.75,110) .. controls (388.24,110) and (393.5,115.26) .. (393.5,121.75) .. controls (393.5,128.24) and (388.24,133.5) .. (381.75,133.5) .. controls (375.26,133.5) and (370,128.24) .. (370,121.75) -- cycle ;
%Shape: Circle [id:dp34607582518900304] 
\draw  [fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=1 ] (388,63.75) .. controls (388,57.26) and (393.26,52) .. (399.75,52) .. controls (406.24,52) and (411.5,57.26) .. (411.5,63.75) .. controls (411.5,70.24) and (406.24,75.5) .. (399.75,75.5) .. controls (393.26,75.5) and (388,70.24) .. (388,63.75) -- cycle ;
%Shape: Circle [id:dp9051799107756784] 
\draw  [fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=1 ] (409.75,37.25) .. controls (409.75,30.76) and (415.01,25.5) .. (421.5,25.5) .. controls (427.99,25.5) and (433.25,30.76) .. (433.25,37.25) .. controls (433.25,43.74) and (427.99,49) .. (421.5,49) .. controls (415.01,49) and (409.75,43.74) .. (409.75,37.25) -- cycle ;
%Shape: Circle [id:dp9886972020516329] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (412,152.75) .. controls (412,146.26) and (417.26,141) .. (423.75,141) .. controls (430.24,141) and (435.5,146.26) .. (435.5,152.75) .. controls (435.5,159.24) and (430.24,164.5) .. (423.75,164.5) .. controls (417.26,164.5) and (412,159.24) .. (412,152.75) -- cycle ;
%Shape: Circle [id:dp22836829760633237] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (438.75,122.25) .. controls (438.75,115.76) and (444.01,110.5) .. (450.5,110.5) .. controls (456.99,110.5) and (462.25,115.76) .. (462.25,122.25) .. controls (462.25,128.74) and (456.99,134) .. (450.5,134) .. controls (444.01,134) and (438.75,128.74) .. (438.75,122.25) -- cycle ;
%Shape: Circle [id:dp43319006708215224] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (462.75,156) .. controls (462.75,149.51) and (468.01,144.25) .. (474.5,144.25) .. controls (480.99,144.25) and (486.25,149.51) .. (486.25,156) .. controls (486.25,162.49) and (480.99,167.75) .. (474.5,167.75) .. controls (468.01,167.75) and (462.75,162.49) .. (462.75,156) -- cycle ;
%Straight Lines [id:da922216620539261] 
\draw    (330.75,130.5) -- (344.75,153) ;
%Straight Lines [id:da07599765878555509] 
\draw    (330.75,130.5) -- (369.5,127) ;
%Straight Lines [id:da5784724259070599] 
\draw    (369.5,127) -- (344.75,153) ;
%Straight Lines [id:da49580597577586305] 
\draw    (381.75,110) -- (399.75,75.5) ;
%Straight Lines [id:da3412224937379251] 
\draw    (392.5,128) -- (414.5,144) ;
%Straight Lines [id:da17841804218848467] 
\draw    (409.5,56) -- (421.5,49) ;
%Straight Lines [id:da29605259803919903] 
\draw    (436.5,67) -- (421.5,49) ;
%Shape: Circle [id:dp046308926182984766] 
\draw  [fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=1 ] (430,73.75) .. controls (430,67.26) and (435.26,62) .. (441.75,62) .. controls (448.24,62) and (453.5,67.26) .. (453.5,73.75) .. controls (453.5,80.24) and (448.24,85.5) .. (441.75,85.5) .. controls (435.26,85.5) and (430,80.24) .. (430,73.75) -- cycle ;
%Straight Lines [id:da998437851451426] 
\draw    (430.5,144) -- (450.5,134) ;
%Straight Lines [id:da6916101301583182] 
\draw    (450.5,134) -- (462.75,156) ;
%Straight Lines [id:da7736086289511626] 
\draw    (432.5,158) -- (462.75,156) ;
%Curve Lines [id:da9306114377774204] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (484.5,149) .. controls (524.5,119) and (488.75,71) .. (453.5,73.75) ;




\end{tikzpicture}


==> figures/old-figs/multiRelGraphs.tex <==

\begin{tikzpicture}[%
 block/.style={rectangle, fill=gray, text centered, minimum height=8mm, rounded corners=1mm}
        ,my line style1/.style={ draw=purple,thick}
        ,my line style2/.style={ draw=blue,thick}
        ,my line style3/.style={ draw=black,dashdotted,thick}
        ,every label/.append style = {label distance=1pt, inner sep=1pt, 
                             align=left, font=\tiny}
        %,every edge/.style={my line style}
        ,my edge/.style={my line style, mylabel=#1}
        ,my curved edge/.style n args={4}{my line style, out=#1, in=#2, looseness=#3, mylabel=#4}
        ,edge1/.style={my line style1,dashed}
        ,mylabel1/.style={my label style{#1}}
        ,edge2/.style={my line style2, densely dotted}
        ,edge3/.style={my line style3}
        ,mylabel/.style={edge node={node[my label style]{#1}}}]
  % Place super peers and connect them
\foreach \distxbetweengraphs\distybetweengraphs\graphid in {{0/2/0},{4/2/1},{2/0/2}}
  \foreach \place/\name in {{(0+\distxbetweengraphs,-0.5+\distybetweengraphs)/ar\graphid}, {(0.5+\distxbetweengraphs,0.3+\distybetweengraphs)/br\graphid}, {(0+\distxbetweengraphs,1+\distybetweengraphs)/cr\graphid}, {(-0.5+\distxbetweengraphs,0.6+\distybetweengraphs)/dr\graphid},
           {(-0.5+\distxbetweengraphs,0+\distybetweengraphs)/er\graphid}}
    \node[superpeers] (\name) at \place {};
  
   %
   % Place normal peers
  
   \foreach \source/\dest in {ar0/bd0, ar0/cr0, ad0/dd0,bd0/cd0,  br0/cr0, cr0/dr0,ad0/ed0,dr0/er0,
   cd0/dd0,dr0/ad0}
    \path (\source) edge[edge1] (\dest);
    \foreach \source/\dest in {ar1/er1,bd1/dd1,cd1/ed1, cr1/dr1,bd1/ed1,dd1/er1,
   cr1/dr1,dr1/bd1,br1/bd1,ed1/ad1}
    \path (\source) edge[edge2] (\dest);
    \foreach \source/\dest in {ar2/er2,bd2/dd2,cd2/ed2, cr2/dr2,bd2/ed2, cr2/dr2,ad2/ed2,dr2/er2,
   cd2/dd2,dr2/ad2,br2/ar2}
    \path (\source) edge[edge3] (\dest);
   %%%%%%%%
   % Legends
    \node[superpeers,label={[font=\small]0: : Democrat}] (d) at (0,4.1) {};
    \node[peers,label={[font=\small]0: : Republican}] (r) at (0,3.6) {};
   %\node[legendsp] at  {\small{Democrats}};
   %\node[legendp] at  {\small{Rebublicans}};
   %\node[legend_general] at (0,4) {\small{\textsc{Skype-topology}}};
    \node at (3,3.6) (nA) {};
    \node[label={[font=\small]0: : Friends}] at (4,3.6) (nB) {};
    \path (nA) edge[edge1] (nB);
    \node at (3,3.9) (nA1) {};
    \node[label={[font=\small]0: : Same soccer team}] at (4,3.9) (nB1) {};
    \path (nA1) edge[edge2] (nB1);
    \node at (3,4.2) (nA2) {};
    \node[label={[font=\small]0: : Coworkers}] at (4,4.2) (nB2) {};
    \path (nA2) edge[edge3] (nB2);
\end{tikzpicture}

==> figures/old-figs/multiRelGraphsnew.tex <==

\begin{tikzpicture}[%
 block/.style={rectangle, fill=gray, text centered, minimum height=8mm, rounded corners=1mm}
        ,my line style1/.style={ draw=purple,thick}
        ,my line style2/.style={ draw=blue,thick}
        ,my line style3/.style={ draw=black,dashdotted,thick}
        ,every label/.append style = {label distance=1pt, inner sep=1pt, 
                             align=left, font=\tiny}
        %,every edge/.style={my line style}
        ,my edge/.style={my line style, mylabel=#1}
        ,my curved edge/.style n args={4}{my line style, out=#1, in=#2, looseness=#3, mylabel=#4}
        ,edge1/.style={my line style1,dashed}
        ,mylabel1/.style={my label style{#1}}
        ,edge2/.style={my line style2, densely dotted}
        ,edge3/.style={my line style3}
        ,mylabel/.style={edge node={node[my label style]{#1}}}]
  % Place super peers and connect them
\foreach \distxbetweengraphs\distybetweengraphs\graphid in {{0/2/0},{4/2/1},{2/0/2}}
  \foreach \place/\name in {{(0+\distxbetweengraphs,-0.5+\distybetweengraphs)/ar\graphid}, {(0.5+\distxbetweengraphs,0.3+\distybetweengraphs)/br\graphid}, {(0+\distxbetweengraphs,1+\distybetweengraphs)/cr\graphid}, {(-0.5+\distxbetweengraphs,0.6+\distybetweengraphs)/dr\graphid},
           {(-0.5+\distxbetweengraphs,0+\distybetweengraphs)/er\graphid}}
    \node[superpeers] (\name) at \place {};
  
   %
   % Place normal peers
  \foreach \distxbetweengraphs\distybetweengraphs\graphid in {{0/2/0},{4/2/1},{2/0/2}}
  \foreach\place/\name  in {{(1+\distxbetweengraphs,-0.5+\distybetweengraphs)/ad\graphid}, {(1.5+\distxbetweengraphs,0+\distybetweengraphs)/bd\graphid}, {(0.6+\distxbetweengraphs,1.2+\distybetweengraphs)/cd\graphid}, {(2+\distxbetweengraphs,1+\distybetweengraphs)/dd\graphid},
                        {(2+\distxbetweengraphs,0+\distybetweengraphs)/ed\graphid}}
    \node[peers] (\name) at \place {};
   
   %
   \foreach \source/\dest in {ar0/bd0, ar0/cr0, ad0/dd0,bd0/cd0,  br0/cr0, cr0/dr0,ad0/ed0,dr0/er0,
   cd0/dd0,dr0/ad0}
    \path (\source) edge[edge1] (\dest);
    \foreach \source/\dest in {ar1/er1,bd1/dd1,cd1/ed1, cr1/dr1,bd1/ed1,dd1/er1,
   cr1/dr1,dr1/bd1,br1/bd1,ed1/ad1}
    \path (\source) edge[edge2] (\dest);
    \foreach \source/\dest in {ar2/er2,bd2/dd2,cd2/ed2, cr2/dr2,bd2/ed2, cr2/dr2,ad2/ed2,dr2/er2,
   cd2/dd2,dr2/ad2,br2/ar2}
    \path (\source) edge[edge3] (\dest);
   %%%%%%%%
   % Legends
    \node[superpeers,label={[font=\small]0: : Democrat}] (d) at (0,4.1) {};
    \node[peers,label={[font=\small]0: : Republican}] (r) at (0,3.6) {};
   %\node[legendsp] at  {\small{Democrats}};
   %\node[legendp] at  {\small{Rebublicans}};
   %\node[legend_general] at (0,4) {\small{\textsc{Skype-topology}}};
    \node at (3,3.6) (nA) {};
    \node[label={[font=\small]0: : Friends}] at (4,3.6) (nB) {};
    \path (nA) edge[edge1] (nB);
    \node at (3,3.9) (nA1) {};
    \node[label={[font=\small]0: : Same soccer team}] at (4,3.9) (nB1) {};
    \path (nA1) edge[edge2] (nB1);
    \node at (3,4.2) (nA2) {};
    \node[label={[font=\small]0: : Coworkers}] at (4,4.2) (nB2) {};
    \path (nA2) edge[edge3] (nB2);
\end{tikzpicture}

==> figures/old-figs/network.tex <==
\begin{tikzpicture}[]
\clip (0,0) rectangle (8.0,8.0);
\Vertex[x=2.868,y=5.518,size=0.5,color=blue,opacity=0.7,label=CA,position=below]{a}
\Vertex[x=1.000,y=7.000,size=0.5,color=blue,opacity=0.7,label=CA,position=below]{b}
\Vertex[x=5.006,y=5.387,size=0.5,color=red,opacity=0.7,label=Claire,position=below]{c}
\Vertex[x=6.858,y=3.552,size=0.5,color=blue,opacity=0.7,label=Dennis,position=below]{d}
\Vertex[x=7.000,y=6.419,size=0.5,color=red,opacity=0.7,label=Esther,position=below]{e}
\Vertex[x=3.698,y=2.808,size=0.5,color=blue,opacity=0.7,label=Frank,position=below]{f}
\Vertex[x=5.551,y=1.000,size=0.5,color=blue,opacity=0.7,label=George,position=below]{g}
\Edge[,lw=1.0,bend=-8.531,Direct](a)(b)
\Edge[,lw=1.0,bend=-8.531,Direct](a)(c)
\Edge[,lw=3.0,bend=-8.531,Direct](c)(d)
\Edge[,lw=3.0,bend=-8.531,Direct](d)(e)
\Edge[,lw=3.0,bend=-8.531,Direct](e)(c)
\Edge[,lw=1.0,bend=-8.531,Direct](c)(f)
\Edge[,lw=3.0,bend=-8.531,Direct](f)(a)
\Edge[,lw=1.0,bend=-8.531,Direct](f)(g)
\Edge[,lw=1.0,bend=-8.531,Direct](g)(g)
\Edge[,lw=1.0,bend=-8.531,Direct](g)(d)
\end{tikzpicture}
